Efficient Optimization for Rank-based Loss Functions

The accuracy of information retrieval systems is often measured using complex loss functions such as the average precision (AP) or the normalized discounted cumulative gain (NDCG). Given a set of positive and negative samples, the parameters of a retrieval system can be estimated by minimizing these loss functions. However, the non-differentiability and non-decomposability of these loss functions does not allow for simple gradient based optimization algorithms. This issue is generally circumvented by either optimizing a structured hinge-loss upper bound to the loss function or by using asymptotic methods like the direct-loss minimization framework. Yet, the high computational complexity of loss-augmented inference, which is necessary for both the frameworks, prohibits its use in large training data sets. To alleviate this deficiency, we present a novel quicksort flavored algorithm for a large class of non-decomposable loss functions. We provide a complete characterization of the loss functions that are amenable to our algorithm, and show that it includes both AP and NDCG based loss functions. Furthermore, we prove that no comparison based algorithm can improve upon the computational complexity of our approach asymptotically. We demonstrate the effectiveness of our approach in the context of optimizing the structured hinge loss upper bound of AP and NDCG loss for learning models for a variety of vision tasks. We show that our approach provides significantly better results than simpler decomposable loss functions, while requiring a comparable training time.

==> sections/additional.tex <==
The computation of the optimal interleaving rank for a particular negative
sample requires us to maximize the discrete function $f_j(i)$ over the domain $i \in \{1,\cdots,|{\cal P}|\}$ (or possibly its subdomain). Yue {\em et al.\ }\cite{yuesigir07}
use a simple linear algorithm for this step, which takes $O(|{\cal P}|)$ time. In contrast, we propose a more efficient algorithm to maximize
$\delta_j(\cdot)$, which exploits the special structure of this discrete function. This will not bring improvement in the worst-case complexity but it adds another speed-up and is interesting conceptually.

Before we describe our efficient algorithm in detail, we require the definition of a unimodal function. A discrete function $f:\{1,\cdots,p\} \leftarrow \mathbb{R}$
is said to be unimodal if and only if there exists a $k \in \{1,\cdots,p\}$ such that
\begin{eqnarray}
&&f(i) \leq f(i+1), \forall i \in \{1,\cdots,k-1\}, \nonumber \\
&&f(i-1) \geq f(i), \forall i \in \{k+1,\cdots,p\}.
\end{eqnarray}
In other words, a unimodal discrete function is monotonically non-decreasing in the interval $[1,k]$ and monotonically non-increasing in the interval $[k,p]$.
The maximization of a unimodal discrete function over its domain $\{1,\cdots,p\}$ simply requires us to find the index $k$ that satisfies the above
properties. The maximization can be performed efficiently, in $O(\log(p))$ time, using binary search.

We are now ready to state the main result that allows us to compute the optimal interleaving rank of a negative sample efficiently.
\begin{proposition}\label{prop:unimodal}\setcounter{foo}{\value{theorem}}
%\item 
The discrete function $f_j(i)$, induced by $\Delta_{AP}$, is unimodal in the domain $\{1,\cdots,p\}$, where
$p = \min\{|{\cal P}|,j\}$.
%\label{prop:unimodal}
\end{proposition}

The proof of the above proposition is provided in Appendix \ref{sec:lossprops}.

\begin{algorithm}[h]
\caption{\em Efficient search for the optimal interleaving rank of a negative sample.} \label{alg2}
\SetAlgoLined
\DontPrintSemicolon

\nonl 
{\bf Input:} $\{f_j(i),i=1,\cdots,|{\cal P}|\}$. \\
\vspace{-10pt}\; 

$p = \min\{|{\cal P}|,j\}$\;
Compute an interleaving rank $i_1$ as
\begin{equation}
i_i = \argmax_{i \in \{1,\cdots,p\}} f_j(i).
\end{equation}\vspace{-10pt}\;
Compute an interleaving rank $i_2$ as
\begin{equation}
i_2 = \argmax_{i \in \{p+1,\cdots,|{\cal P}|\}} f_j(i).
\end{equation}\vspace{-10pt}\;
Compute the optimal interleaving rank $opt_j$ as
\begin{equation}
opt_j = \left\{
\begin{array}{cl}
i_1 & \mbox{if } f_j(i_1) \geq f_j(i_2), \\
i_2 & \mbox{otherwise}.
\end{array}
\right.
\end{equation}

\end{algorithm}
Using the above proposition, the discrete function $f_j(i)$ can be optimized over the domain $\{1,\cdots,|{\cal P}|\}$ efficiently
as described in Algorithm~\ref{alg2}. Briefly, our efficient search algorithm finds
an interleaving ranking $i_1$ over the domain $\{1,\cdots,p\}$, where
$p$ is set to $\min\{|{\cal P}|,j\}$ in order to ensure that the function $f_j(\cdot)$ is unimodal (step 2 of Algorithm~\ref{alg2}).
Since $i_1$ can be computed using binary search, the computational complexity of this step is $O(\log(p))$.
Furthermore, we find an interleaving ranking $i_2$ over the domain $\{p+1,\cdots,|{\cal P}|\}$ (step 3 of Algorithm~\ref{alg2}).
Since $i_2$ needs to be computed using linear search, the computational complexity of this step is $O(|{\cal P}|-p)$ when $p < |{\cal P}|$ and $0$ otherwise.
The optimal interleaving ranking $opt_j$ of the negative sample ${\bf x}_j$ can then be computed by comparing the values of
$f_j(i_1)$ and $f_j(i_2)$ (step 4 of Algorithm~\ref{alg2}).

Note that, in a typical training data set, the negative samples significantly outnumber the positive samples, that is, $|{\cal N}| \gg |{\cal P}|$.
For all the negative samples ${\bf x}_j$ where $j \geq |{\cal P}|$, $p$ will be equal to $|{\cal P}|$. Hence, the maximization of $f_j(\cdot)$ can
be performed efficiently over the entire domain $\{1,\cdots,|{\cal P}|\}$ using binary search in $O(\log(|{\cal P}|))$ as opposed to the
$O(|{\cal P}|)$ time suggested in~\cite{yuesigir07}.


